Quantum Optimal Control Theory of Harmonic Generation

A new method for controlling harmonic generation, in the framework of quantum optimal control theory (QOCT), is developed. The problem is formulated in the frequency domain using a new maximization functional. The relaxation method is used as the optimization procedure. The new formulation is generalized to other control problems with requirements in the frequency domain. The method is applied to several simple problems. The results are analysed and discussed. General conclusions on harmonic generation mechanisms are obtained.

==> HGCnum.tex <==
%\documentclass[a4paper]{article}
%
%\usepackage{amsmath}
%\usepackage{graphicx}
%\input{mymathcommands}
%\input{quantumcommands}
%\input{mytextcommands}
%
%\newcommand{\epsw}{\bar{\epsilon}(\omega)}
%\newcommand{\etaw}{\bar{\eta}(\omega)}
%\newcommand{\muw}{\overline{\exval{\operator{\mu}}}(\omega)}
%\newcommand{\Ow}{\overline{\exval{\operator{O}}}(\omega)}
%\newcommand{\Oaw}{\overline{\exval{\operator{O}_a}}(\omega)}
%
%\newcommand{\feps}{f_{\epsilon}(\omega)}
%\newcommand{\tfeps}{\tilde{f}_{\epsilon}(\omega)}
%\newcommand{\fmu}{f_{\mu}(\omega)}
%\newcommand{\tfmu}{\tilde{f}_{\mu}(\omega)}
%\newcommand{\fO}{f_{O}(\omega)}
%\newcommand{\tfO}{\tilde{f}_{O}(\omega)}
%
%\newcommand{\evmu}{\exval{\operator{\mu}}\!(t)}
%
%\newcommand{\opq}[1]{\operator{q}^{(#1)}}
%\newcommand{\opdo}[1]{\operator{d}_o^{(#1)}}
%\newcommand{\opdO}[1]{\operator{d}_O^{(#1)}}
%\newcommand{\opO}[1]{\operator{O}^{(#1)}}
%\newcommand{\opmu}[1]{\operator{\mu}^{(#1)}}
%\newcommand{\muwn}[1]{\overline{\exval{\operator{\mu}^{(#1)}}}(\omega)}
%
%\begin{document}
\section{The performance of the Hamiltonian operations}
The Hamiltonian operations in the problems that depend on a spatial variable $x$, were performed using the Fourier grid method (see~\cite{TDmethods}). The operation of the $x$ dependent terms in the Hamiltonian is performed in the $x$ domain, and the operation of the $p$ dependent term, \ie the kinetic energy, is performed in the $p$ domain.

\section{The choice of the $x$ grid}
The $x$ grids of the various problems are equidistant grids. The distance between neighbouring points in the $x$ domain \text{$[x_{min}, x_{max})$} is:
\[
	\Delta x = \frac{x_{max}-x_{min}}{N_{grid}}
\]
where $N_{grid}$ is the number of grid points.

The $x$ domain is chosen to satisfy: 
\begin{align}
	& V(x_{min}) = V(x_{max}) \label{eq:Vmm}\\
	& V_{max} = \frac{p_{max}^2}{2m} = \frac{\pi^2}{2m\,\Delta x^2} \label{eq:VmTm}
\end{align}
where $V_{max}$ is the maximal $V(x)$, $p_{max}$ is the maximal momentum, and $m$ is the mass, or reduced mass.  \eqref{eq:VmTm} makes the maximal $V(x)$ possible, equal to the maximal kinetic energy possible.

\section{The approximation of the cosine transform}
The cosine transform was approximated using a discrete-cosine-transform that include the boundaries of the domain. It is sometimes referred as the DCT of the first kind (DCT-I, see~\cite{DCT}). The DCT-I of $N_t$ equidistant time points:
\[
	t_i, \qquad i=0,1,\ldots,N_t-1
\]
is defined as:
\begin{align}
	& \bar{g}(\omega_j) = \sqrt{\frac{2}{N_t-1}}\sum_{i=0}^{N_t-1}\frac{1}{h_i} g(t_i)\cos\left(\frac{ij\pi}{N_t-1}\right), & &j=0,1,\ldots,N_t-1 \label{eq:DCT}\\
	& h_i =
	\begin{cases}
		2 & \qquad i=0 \text{ or } i=N_t-1 \\
		1 & \qquad 1\leq i\leq N_t-2
	\end{cases} \label{eq:hdef}
\end{align}

Using this convention, DCT-I is its own inverse. In order to be consistent with the continuous formulation, the direct transform is multiplied by the factor: $T/\sqrt{(N_t-1)\pi}$. The inverse transform is divided by this factor. This is also necessary for another reason: when using Eq.~\eqref{eq:DCT} as is, the definition of the spectral function $\bar{g}(\omega)$, represented by the transform, varies with the sampling frequency. This is corrected by the insertion of the factor. 

The computation of the DCT-I is performed by the FFT of the ``folded'' function (see~\cite{DCT}).

\section{The computation of $J$}
The gradient and relaxation methods involve the computation of the functional $J$, during the search for an appropriate parameter $K$. In order that these methods will be successful, it is important to compute the integrals in $J$ as accurately as possible. The accuracy of the numerical integration should be the same as that of the propagator.

The integration of the $\omega$ dependent functions is performed like in the DCT-I. This is consistent with the accuracy of the $\omega$ grid.

The integration of the $t$ dependent functions is performed by utilizing the internal Chebyshev time points of every time step. We describe here the integration method.

Consider a time step with the boundaries: \text{$[t_n, t_{n+1}]$}. Within the time interval, there are $N_c$ internal points --- the boundary including Chebyshev points:
\begin{align}
	& t_k = t_n + \frac{\Delta t}{2}(1-y_k) &  \label{eq:Chebpt}\\
	& y_k = \cos\left(\frac{k\pi}{N_c - 1}\right) & \qquad k=0,1,\ldots ,N_c - 1 \label{eq:Chebpy}
\end{align}
where $\Delta t = t_{n+1}-t_n$.

An arbitrary time-dependent function $g(t)$ defined in the interval may be approximated by a truncated Chebyshev series:
\begin{equation}\label{eq:chebser}
	g(t) \approx \sum_{m=0}^{N_c-1}a_m T_m(y) \qquad\qquad y=\frac{-2t+t_n+t_{n+1}}{\Delta t}
\end{equation}
where the $T_m(y)$ are the Chebyshev polynomials. The $a_m$ are given by:
\begin{equation}\label{eq:chebcoef}
	a_m = -\frac{2}{(N_c-1)h_m}\sum_{k=0}^{N_c-1}\frac{1}{h_k}g(t_k)\cos\left(\frac{km\pi}{N_c-1}\right)
\end{equation}
where $h_i$ is defined by Eq.~\eqref{eq:hdef}.

The integration of $g(t)$ over the interval may be approximated using \eqref{eq:chebser}:
\begin{align}
	& \int_{t_n}^{t_{n+1}}g(t)\,dt\approx-\frac{\Delta t}{2}\sum_{m=0}^{N_c-1}a_m\int_{-1}^{1}T_m(y)\,dy=-\Delta t \sum_{m=0}^{N_c-1}a_m c_m \label{eq:sumac}\\
	& c_m = 
	\begin{cases}
		-\frac{1}{m^2-1} & \qquad m \text{ even} \\
		0 & \qquad m \text{ odd}
	\end{cases}
\end{align}
The integration of the $T_m(y)$ is performed analytically.

Inserting \eqref{eq:chebcoef} into \eqref{eq:sumac}, we obtain:
\begin{align}
	& \int_{t_n}^{t_{n+1}}g(t)\,dt\approx \Delta t \sum_{k=0}^{N_c-1}w_k g(t_k) \label{eq:chebint}\\
	& w_k \equiv \frac{2}{(N_c-1)h_k}\sum_{m=0}^{N_c-1}\frac{1}{h_m}c_m\cos\left(\frac{km\pi}{N-1}\right) \label{eq:wdef}
\end{align}
The $w_k$ are the integration weights of the $t_k$, for $N_c$ Chebyshev points. They are independent of $\Delta t$. The expression for $w_k$ is just a DCT-I of $c_m$, within a factor, and an additional small difference (compare Eq.~\eqref{eq:DCT}). It may be computed efficiently, using a FFT. If all time steps have the same internal structure, the computation of the $w_k$ has to be performed only once.

\section{The tolerance parameters}
The tolerance parameter of the convergence in the optimization procedures is the maximal allowed relative difference of the field at the end of the process. Let us denote the tolerance parameter of the optimization as $\tau$. For the problems with the regular $J_{penal}$ (Eq.~\eqref{eq:Jpenals2s}), the convergence condition is:
\begin{align}
	& \frac{\Vert \vec{\epsilon}^{\text{ }new}-\vec{\epsilon}^{\text{ }old} \Vert}{\Vert \vec{\epsilon}^{\text{ }new} \Vert}<\tau \label{eq:tolt}\\
	& \vec{\epsilon} \equiv
	\begin{bmatrix}
		\epsilon(t_0)\\
		\epsilon(t_1)\\
		\vdots\\
		\epsilon(t_{N_t-1})
	\end{bmatrix}
\end{align}
For the problems with the new $J_{penal}$ (Eq.~\eqref{eq:Jpenalw}), the condition is:
\begin{align}
	& \frac{\Vert \vec{\bar\epsilon}^{\text{ }new}-\vec{\bar\epsilon}^{\text{ }old} \Vert}{\Vert \vec{\bar\epsilon}^{\text{ }new} \Vert}<\tau \label{eq:tolw}\\
	& \vec{\bar\epsilon} \equiv
	\begin{bmatrix}
		\bar\epsilon(\omega_0)\\
		\bar\epsilon(\omega_1)\\
		\vdots\\
		\bar\epsilon(\omega_{N_t-1})
	\end{bmatrix}
\end{align}

We also used a tolerance parameter for the propagator, unlike in the attached article. We allowed the possibility of more than one iteration in all time-steps, and not only in the first one (for efficiency, the average number of iterations should not exceed $1$ too much; this may be achieved by choosing a sufficiently small $\Delta t$, and a sufficiently large $N_c$). Let us denote the tolerance parameter of the propagator as $\zeta$. The convergence condition is:
\begin{equation}
	\frac{\Vert \mathbf{u}^{new}-\mathbf{u}^{old} \Vert}{\Vert \mathbf{u}^{old} \Vert}<\zeta
\end{equation}
where $\mathbf{u}$ is the solution vector at the edge of the time step interval. We take: \text{$\zeta=10^{-3}\,\tau$}. 

%
%	\begin{thebibliography}{999}
%		\input{HGCbib}
%	\end{thebibliography}
%			
%
%\end{document}

%The discrete Fourier transform (DFT) is based on the approximation of a function defined in a limited interval, by a truncated Fourier series; an arbitrary function $g(t)$, defined in the interval: $[0,\; T]$, is spanned by a finite series of the following form:
%\begin{equation}\label{eq:Fser}
%	g(t) = \frac{1}{\sqrt{N}}\sum_{n=0}^{N-1} a_n\exp(in\,\Delta\omega\,t), \qquad t\in[0,\;T], \qquad \Delta\omega \equiv \frac{2\pi}{T}
%\end{equation}
%where the $a_n$ are Fourier coefficients. $N$ is the number of equidistant sampling points of $g(t)$, where $\Delta t=T/N$. The actual function approximated by the Fourier series is a periodical function, defined as:
%\begin{equation}\label{eq:Fser2}
%	\tilde{g}(t) = \frac{1}{\sqrt{N}}\sum_{n=0}^{N-1} a_n\exp(in\,\Delta\omega\,t), \qquad t\in(-\infty,\infty)
%\end{equation}
%It satisfies: $\tilde{g}(t)=\tilde{g}(t+T)$. 
%
%The Fourier series is an adequate representation of $\tilde{g}(t)$, if the maximal frequency of $\tilde{g}(t)$ do not exceed $(N-1)\Delta\omega$. Otherwise, the \emph{ringing phenomenon} will appear --- we will observe oscillations throughout the spectral function.
%
%The problem starts when $g(0)\neq g(T)$; then there is a discontinuity in $\tilde{g}(t)$ in the points:
%\[
%	t=mT \qquad\qquad m=\ldots,-1,0,1,\ldots
%\]
%The discontinuity contains functions of very high frequencies, and the ringing phenomenon will be observed.
%
%One possible solution is to use the discrete cosine transform (DCT) instead of the DFT; the DCT is based on ``folding'' $g(t)$, and performing a Fourier transform on the folded function.

